Skimming and Scanning for Untrimmed Video Action Recognition

Video action recognition (VAR) is a primary task of video understanding, and untrimmed videos are more common in real-life scenes. Untrimmed videos have redundant and diverse clips containing contextual information, so sampling dense clips is essential. Recently, some works attempt to train a generic model to select the N most representative clips. However, it is difficult to model the complex relations from intra-class clips and inter-class videos within a single model and fixed selected number, and the entanglement of multiple relations is also hard to explain. Thus, instead of "only look once", we argue "divide and conquer" strategy will be more suitable in untrimmed VAR. Inspired by the speed reading mechanism, we propose a simple yet effective clip-level solution based on skim-scan techniques. Specifically, the proposed Skim-Scan framework first skims the entire video and drops those uninformative and misleading clips. For the remaining clips, it scans clips with diverse features gradually to drop redundant clips but cover essential content. The above strategies can adaptively select the necessary clips according to the difficulty of the different videos. To trade off the computational complexity and performance, we observe the similar statistical expression between lightweight and heavy networks, thus it supports us to explore the combination of them. Comprehensive experiments are performed on ActivityNet and mini-FCVID datasets, and results demonstrate that our solution surpasses the state-of-the-art performance in terms of both accuracy and efficiency.

==> discussion.tex <==
\label{sec:discussion}

\paragraph{Metrics for approximate the information gain}
Considering that various metrics are used to measure the distance between two distributions, we use these metrics instead of JS divergence to approximate the information gain. We choose two famous metrics: KL Divergence and Wasserstein Distance. Due to the asymmetry of KL divergence, it has relatively low performance compared to JS divergence. At the same time, Wasserstein Distance can reach a similar accuracy as the JS divergence but need a lot of additional clips as the recompense. Besides, the computation cost of Wasserstein Distance is far more than the JS divergence. Thus, we finally choose the JS divergence to approximate the information gain.


\paragraph{Different distinguishing methods for unannotated clips}
We explore some other approaches for the unannotated clip classifier, and analyze on their schemes.
\begin{enumerate}
    \item Combine the binary classifier and clip-level feature classifier into training together, as multi-task learning. However, the combined loss does not boost the performance but reduces the corresponding performance.
    \item To the feature classifier of N class, regard the unannotated clips as the N+1 class to update the feature classifier. Thus both unannotated clips and annotated clips feed into the feature classifier for training. However, the unannotated clips accounted for a large proportion of whole clips, leading to a severe long-tail distribution problem. Thus the N+1 feature classifier does not give a good performance.
    \item Considering the different effects between mistaking the unannotated clips as the annotated clips and mistaking the annotated clips as the unannotated clips, we adjust the binary weight cross-entropy loss. However, we find that the adjustment of weight will always hurt the overall binary classification. Thus, we keep the original binary classification loss.
\end{enumerate}




==> motivation.tex <==


\paragraph{Observation of Entropy Distribution for skimming} In Fig.~\ref{fig:entropy}(a), we analyze the statistic of the entropy distribution of positive clips and negative clips. Positive clips mean their predicted label in clip-level is the same as the label of videos, which is favorable to the final prediction. In contrast, negative clips are the opposite. Interestingly, we find that when entropy is small, the number of positive clips far exceeds false clips. As entropy increases, the proportion of negative clips increases and exceeds positive clips around threshold 0.6. Thus, we could initially drop many negative clips with a proper entropy threshold, with a slight loss of positive clips. Besides, with the four visualization clips in Fig.~\ref{fig:entropy}(a), we find the high entropy clips are always uninformative, even when they are the positive clips. Therefore, the loss of those positive clips with high entropy can be ignored.

\begin{figure}[!h]
\centering % 图片居中
\includegraphics[width = 8.5cm]{latex/pic/pic_sample.png}
\caption{There are the selected clips of a video on "Cheerleading" of 159 clips under our strategy and Scsampler. Due to the limited space, we only show 5 of 10 clips here. We show the first frame of these clips for each clip and present the clips' index and clip-level predicted label. In scsampler, they only pay attention to the "Tumbling" clips, thus misjudged as "Tumbling". While in our strategy, we select clips not only "Tumbling" but also "Cheerleading", thus comprehensively make the correct prediction.}
\label{fig:compare_sample}
\end{figure}

\paragraph{Motivation of scanning with JS Divergence}
In Fig.~\ref{fig:compare_sample}, we could find that in Scsampler, it misleads the prediction because it only catches the attention on clips with "Tumbling" action but ignore the "Cheerleading" clips, due to only dependent on clips' saliency. Considering the diverse information among the videos, we propose to cover the videos' complete information. As shown in Fig.~\ref{fig:entropy}(b), this is a video about sailing, while there are also many other similar clips but different actions in this video, such as windsurfing, scuba diving, even beer pong. To cover the whole information, we will obtain all these representative meaningful clips with the proposed scanning selection with JS divergence and then combine it to consider comprehensively to decide the video's final class.  


